FusionPainting: Multimodal Fusion with Adaptive Attention for 3D Object Detection

Accurate detection of obstacles in 3D is an essential task for autonomous driving and intelligent transportation. In this work, we propose a general multimodal fusion framework FusionPainting to fuse the 2D RGB image and 3D point clouds at a semantic level for boosting the 3D object detection task. Especially, the FusionPainting framework consists of three main modules: a multi-modal semantic segmentation module, an adaptive attention-based semantic fusion module, and a 3D object detector. First, semantic information is obtained for 2D images and 3D Lidar point clouds based on 2D and 3D segmentation approaches. Then the segmentation results from different sensors are adaptively fused based on the proposed attention-based semantic fusion module. Finally, the point clouds painted with the fused semantic label are sent to the 3D detector for obtaining the 3D objection results. The effectiveness of the proposed framework has been verified on the large-scale nuScenes detection benchmark by comparing it with three different baselines. The experimental results show that the fusion strategy can significantly improve the detection performance compared to the methods using only point clouds, and the methods using point clouds only painted with 2D segmentation information. Furthermore, the proposed approach outperforms other state-of-the-art methods on the nuScenes testing benchmark.

==> 05_ablation_study.tex <==
\section{Ablation Studies} \label{sec:ablation_study}
In this part, we conduct some ablation experiments to analyze individual components of our proposed method, our model are trained and evaluate split \textit{train} and \textit{val} respectively on nuScenes dataset.For Second and PointPillars 3D detector we trained and evaluated with whole dataset,we can see that both of 3D and 2D segmentation information has clearly improved the detect accuracy as showed as Tabel.\ref{tab:ablation_table}(1th and 2th row),Pointpillar received largest mAP(+17.31) and NDS(+8.54) imporved compare with baseline,
while Centerpoint achieved that mAP(+10.49) and NDS(+5.29) imporved with quarter of the training split dataset and eval with whole dataset,Specilly we trained all the model with same config,with 8GPU and 4 batchsize,so the baseline maybe subtle differences between our experiment and official figures.

% \begin{table}[ht!]
% \centering
% 	\resizebox{0.4\textwidth}{!}
% 	{%
% 		\begin{tabular}{l| c| cc }
% 			\hline
% 			%\multicolumn{1}{c }{\multirow{2}{*}{Methods}}& \multicolumn{3}{c}{\textbf{AP(IoU=0.7)}} \\
% 			%\multicolumn{1}{c}{}& \multicolumn{1}{l}{Easy} & \multicolumn{1}{l}{Mod} & \multicolumn{1}{l}{Hard}\\ \hline
% 			Methods & NDS & mAP \\ \hline
%             SECOND baseline &  &    \\
%             SECOND  3dSeg &  &  \\
%             SECOND  2dSeg &  &   \\
%             SECOND  MutiSegFusion  & \textbf{}  & \textbf{}  \\ \hline

%             PointPillar baseline &   57.50 & 43.46 \\
%             PointPillar  3dSeg &  61.59  & 52.18 \\
%             PointPillar  2dSeg & 65.05 & 59.1 & \\
%             PointPillar  MutiSegFusion  & \textbf{} & \textbf{} \\ \hline
            
%             CenterPoint baseline & 60.29  & 51.16 \\
%             CenterPoint 3dSeg & 61.81 & 53.91 &\\
%             CenterPoint 2dSeg &  64.49 &  60.71 & \\
%             CenterPoint MutiSegFusion  & \textbf{} & \textbf{}   \\ \hline
            
% 		\end{tabular}
% 	}
% 	\caption{\normalfont Evaluate the effectiveness of FeatureAgg and MapFusion on public nuScenes validation dataset, where ``w'' stands for ``with''.}
% 	\label{tab:ablation_study}
% \end{table}



%\begin{table}[]
%\centering
%\resizebox{0.5\textwidth}{!}
%{%
%    \setlength{\tabcolsep}{4mm}{
%    \begin{tabular}{lccccc}
%    \hline
%    \textbf{Encoder} & \textbf{3d\_seg} & \textbf{2d\_seg} &\textbf{Attention\_module} &\textbf{mAP} & \textbf{NDS} \\ \hline
%    & & & &50.85 &61.96 \\
%    & \checkmark   & & &54.45  &63.41 \\
%    \textbf{second} &  & \checkmark &  &59.4 &66.03  \\
%    & \checkmark & \checkmark  &  &  &   \\  
%    &\checkmark &\checkmark &\checkmark &  & \\ \hline
%     & & & & 43.46 &57.50  \\
%     & \checkmark &  & &52.18  &61.59  \\
%    \textbf{PointPillars} &  & \checkmark &  &59.1 & 65.05 \\
%     &\checkmark  & \checkmark & &60.77 &66.04  \\ 
%     &\checkmark&\checkmark&\checkmark& & &\hline
%     & & & & 51.16 & 60.29 \\
%     & \checkmark & & & 53.91  &61.81  \\
%    \textbf{CenterPoint} &  &\checkmark &  & 60.71 & 64.49 \\
%     &\checkmark  & \checkmark & & &  \\ 
%     &\checkmark&\checkmark&\checkmark& & &\hline
 %   \end{tabular}
%}
%}
%\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l | lllll}
\hline
\textbf{Baselines} & \textbf{3D Seg} & \textbf{2D Seg} & \textbf{attention-module} & \textbf{mAP(\%)} & \textbf{NDS(\%)} \\ \hline
\multirow{4}{*}{\textbf{Second}}      &  &  &  &50.85 &61.96  \\
                 &\checkmark  &  &  &54.45 (+xxx)  &63.41 (+xxx)  \\
                  &  & \checkmark &  &59.4 (+xxx) &66.03 (+xxx)  \\
                  &\checkmark & \checkmark &  &  &  \\
                  & \checkmark &  \checkmark &  \checkmark &  &  \\ \hline
\multirow{4}{*}{\textbf{PointPilars}} &  &  &  &43.46 &57.50   \\
                      & \checkmark &  &  &52.18 (+xxx)  &61.59 (+xxx)   \\
                     &  & \checkmark  &  &59.10 (+xxx) & 65.05 (+xxx)  \\
                     & \checkmark & \checkmark &  &60.77 (+xxx) &66.04 (+xxx)  \\ 
                    & \checkmark &  \checkmark &  \checkmark &  &  \\ \hline
\multirow{4}{*}{\textbf{CenterPoint}} &  &  &  &51.16 & 60.29 \\
        & \checkmark &  &  &53.91 (+xxx)  &61.81 (+xxx)   \\
        &  & \checkmark &  & 60.71 (+xxx) & 64.49 (+xxx)\\
        & \checkmark  & \checkmark  &   &61.65  & 65.58  \\
         & \checkmark & \checkmark & \checkmark  &  &  \\ \hline
\end{tabular}
}
\caption{\normalfont Ablation experiments of different fusion strategies,3D seg,2D Seg represent  sent 3D and 2D semantic segmentation features with raw point feature  as input data to 3D detector respectively,and attention-module is add adaptive learning weight module to framework,all the experiments on  nuScenes validation dataset}
\label{tab:ablation_table}
\end{table}
